OIM: Oscillator-based Ising Machines for Solving Combinatorial Optimisation Problems

We present a new way to make Ising machines, i.e., using networks of coupled self-sustaining nonlinear oscillators. Our scheme is theoretically rooted in a novel result that establishes that the phase dynamics of coupled oscillator systems, under the influence of sub-harmonic injection locking, are governed by a Lyapunov function that is closely related to the Ising Hamiltonian of the coupling graph. As a result, the dynamics of such oscillator networks evolve naturally to local minima of the Lyapunov function. Two simple additional steps (i.e., adding noise, and turning sub-harmonic locking on and off smoothly) enable the network to find excellent solutions of Ising problems. We demonstrate our method on Ising versions of the MAX-CUT and graph colouring problems, showing that it improves on previously published results on several problems in the G benchmark set. Our scheme, which is amenable to realisation using many kinds of oscillators from different physical domains, is particularly well suited for CMOS IC implementation, offering significant practical advantages over previous techniques for making Ising machines. We present working hardware prototypes using CMOS electronic oscillators.

==> code-inclusion-config.tex <==
\lstloadlanguages{Matlab}
\lstset{language=Matlab,
        frame=single, % Single frame around code
        basicstyle=\scriptsize\ttfamily,
        % keywordstyle=[1]\color{blue}\bf, % Perl functions bold and blue
        keywordstyle=[3]\color{blue}\underbar, % Custom functions underlined and blue
        identifierstyle=, % Nothing special about identifiers                                         
        commentstyle=\usefont{T1}{pcr}{m}{sl}\color{MyDarkGreen}\scriptsize, 
            % Comments are in small dark green courier font
        stringstyle=\color{MyDarkRed}, 
        showstringspaces=false, % Don't put marks in string spaces
        tabsize=4, % 5 spaces per tab
        % 
        % Put standard functions not included in the default language here
        %morekeywords={rand},
        % Put function parameters here
        %morekeywords=[2]{on, off, interp},
        % Put user defined functions here
        %morekeywords=[3]{test},
        %
        morecomment=[l][\color{blue}]{...}, % Line continuation (...) like blue comment
        % numbers=left, % Line numbers on left
        % firstnumber=1, % Line numbers start with line 1
        % numberstyle=\tiny\color{blue}, % Line numbers are blue and small
        % stepnumber=5 % Line numbers go in steps of 5
}

% Creates a new command to include an Matlab script, the first parameter is the
% filename of the script (without .pl), the second parameter is the caption
\newcommand{\matlabscript}[2]{
    \begin{itemize}
    \item[]\lstinputlisting[caption=#2,label=#1]{#1}
    \end{itemize}
}



==> colour-defs.tex <==
% various colours
\definecolor{mylightgrey}{rgb}{0.6,0.6,0.6}
\definecolor{mydarkgrey}{rgb}{0.3,0.3,0.3}
\definecolor{mybrown}{rgb}{0.6,0.2,0}
\definecolor{mylightgreen}{rgb}{0,1,0}
\definecolor{mydarkgreen}{rgb}{0,0.5,0}
\definecolor{MyDarkGreen}{rgb}{0.0,0.4,0.0} % This is the color used for comments
\definecolor{myorange}{rgb}{1,0.4,0}
\definecolor{mypurple}{rgb}{0.8,0,0.8}
\definecolor{MyDarkRed}{rgb}{0.4,0.0,0.0} % This is the color used for strings


==> mechanism.tex <==
\section{Oscillator-based Ising Machines}\seclabel{mechanism}

\begin{figure}[htbp!]
    \centering
    {
        \epsfig{file=figures/fig1.eps, width=\linewidth}
    }
    \caption{Illustration of the basic mechanism of oscillator-based Ising machines:
             (a) oscillator shifts its natural frequency from $f_0$ to $f_1$ under external perturbation;
             (b) oscillator's phase becomes stably locked to the perturbation;
             (c) when the perturbation is at $2f_1$, the oscillator locks to its subharmonic at $f_1$;
             (d) bistable phase locks under subharmonic injection locking;
             (e) coupled subharmonically injection-locked oscillators settle with binary phases
                 representing an optimal spin configuration for an Ising problem.
    \figlabel{fig1}}
\end{figure}

The central mechanism behind the synchronisation of coupled oscillators is
injection locking.
As illustrated in \figref{fig1} (a), when an oscillator with a natural
frequency $f_0$ is injection locked by a small periodic perturbation at a
similar frequency $f_1$, the oscillator changes its frequency to lock to $f_1$.
Its phase also stably locks to that of the perturbation (\figref{fig1} (b)).
More interestingly, when the perturbation is at about twice the oscillator's
frequency, \ie, at $2f_1$, as mentioned in \secref{intro}, subharmonic
injection locking (SHIL) can occur, and the oscillator can develop one of the
two possible responses differing only in the phase by $180^\circ$, as
illustrated in \figref{fig1} (c) and (d).
The perturbation then serves as the SYNC signal for inducing bistability in the
oscillator-based logic latches discussed in \secref{intro}.

If we lower SYNC and reduce the effect of SHIL, due to the
intrinsic noise, the oscillator will have its phase stochastically flipping
between the bistable states --- it ``degrades'' from a binary latch to a binary
random number generator.
Naturally, we can speculate that when several such random number generators are
coupled together, their values will prefer certain configurations over others.
For instance, if two of these oscillators are connected through a resistor,
instead of having four states \{00\}, \{01\}, \{10\}, \{11\} with equal
probabilities, they are more likely to end up in \{00\} and \{11\} --- these
two states become the preferred states of a simple size-2 Ising model.
As illustrated in \figref{fig1} (e), by properly designing the connections in
larger coupled oscillator networks, we can encode more complicated Ising models
for minimisation, thus physically realising larger-scale oscillator-based Ising
machines.

% Note: Here we assume an Ising problem has the following form:
%       min h.'*s + 1/2 * s.'*J*s
%       s.t. s_i = +1 or -1

% for c = 1:n
%     fout(c, 1) = Ac * h(c) * sin(pi*x(c)) ...
%                + Ac * J(c, :) * sin(pi*(x(c) - x));
% end
% fout = (fout - As * sin(2*pi*x))/pi;

To validate this intuition, we need to study the dynamics and steady states of
coupled oscillator networks, and more specifically, what they naturally
minimise.
When a group of oscillators synchronise and their phase pattern stabilises,
people often say a certain ``energy'' reaches a minimum, like a rolling ball
lowering its potential energy by settling towards a valley in a hilly
landscape.
But such an analogy is inaccurate if not erroneous, as a coupled oscillator
system is intrinsically dissipative, and no such conservative ``energy''
exists.
Indeed, as we show in the remainder of this section and prove more rigorously in
\secref{theory}, it is not a physical energy, but a collective global Lyapunov
function that coupled oscillators minimise.
And with the help of SHIL-induced Booleanisation, we can modify this global
Lyapunov function and encode the Ising Hamiltonian in it.

As a start to our analysis, we consider a commonly used macromodel for coupled
oscillators --- the Kuramoto model [][], first proposed by Japanese physicist
Yoshiki Kuramoto.
\begin{equation}\eqnlabel{KuramotoOriginal}
    \frac{d}{dt} \phi_i(t) = - \frac{K}{n} \cdot \sum_{j=1,~j \neq i}^n \sin(\phi_i(t) - \phi_j(t)), \qquad i = 1, \cdots, n,
\end{equation}
where $\{\phi_i\}$ represents the phases of $n$ oscillators; scalar $K$ is the
coupling strength.

The original Kuramoto model describes an oscillator network with all-to-all
connectivity of equal weights.
As we show in more detail in \secref{theory}, this does not have to be the
case; a generalised model can incorporate coefficients $\{J_{ij}\}$\footnote{In
the Ising Hamiltonian \eqnref{IsingH}, $J_{ij}$ is only defined when $i<j$;
here we assume that $J_{ij} = J_{ji}$ for all $i,~j$.} into the connections
between oscillators.
\begin{equation}\eqnlabel{KuramotoTHREE}
	\frac{d}{dt} \phi_i(t) = -K \cdot \sum_{j=1,~j \neq i}^n J_{ij} \cdot \sin(\phi_i(t) - \phi_j(t)).
\end{equation}

This generalised Kuramoto model describes a gradient system []
\cite{smale1961gradient}. % find a better citation
We can assign an ``energy'' function in the following form, and prove that it
is a global Lyapunov function for the system.
\begin{equation}\eqnlabel{E}
	E(\vec\phi(t)) = -K\cdot \sum_{i,j,~i \neq j} J_{ij} \cdot \cos(\phi_i(t) - \phi_j(t)),
\end{equation}
where $\vec\phi(t) = [\phi_1(t),\cdots,\phi_n(t)]^T$.

We observe that $E$ is the summation of $(n^2-n)$ number of $\cos()$ terms.
Among them, for any given $i$, variable $\phi_i$ appears $2\cdot(n-1)$ times --- $(n-1)$ times
as the subtrahend and $(n-1)$ times as the minuend inside the $\cos()$ function.
So if we differentiate $E$ with respect to $\phi_i$, we have
\begin{align}
	\frac{dE(\vec\phi(t))}{d\phi_i(t)} &= -K\cdot \sum_{j=1,~j\neq i}^n J_{ij}
					 \frac{d}{d\phi_i(t)} \left[\cos(\phi_i(t) - \phi_j(t))\right]
	                        -K\cdot \sum_{j=1,~j\neq i}^n J_{ij}
					 \frac{d}{d\phi_i(t)} \left[\cos(\phi_j(t) - \phi_i(t))\right] \\
    &= K\cdot \sum_{j=1,~j\neq i}^n J_{ij}
					 \sin(\phi_i(t) - \phi_j(t))
	                        - K\cdot \sum_{j=1,~j\neq i}^n J_{ij}
					 \sin(\phi_j(t) - \phi_i(t)) \\
    &= K\cdot \sum_{j=1,~j\neq i}^n J_{ij} \cdot 2 \cdot \sin(\phi_i(t) - \phi_j(t)) \\
    &= -2 \cdot \frac{d\phi_i(t)}{dt}.
\end{align}

Therefore, 
\begin{align}
	\frac{dE(\vec\phi(t))}{dt} &= \sum_{i=1}^n \left[ \frac{dE(\vec\phi(t))}{d\phi_i(t)} \cdot
                     \frac{d\phi_i(t)}{dt} \right] \\
	              &= - 2 \cdot \sum_{i=1}^n \left(\frac{d\phi_i(t)}{dt}\right)^2 \leq 0.
\end{align}

As $dE(\vec\phi(t))/dt \leq 0$ for all $\vec\phi$, $E(\vec\phi(t))$ is a
global Lyapunov function, \ie, the coupled oscillator system always tends to
minimise this function as time passes.
The local minima of $E(\vec\phi(t))$ represent the stable equilibria of the
system.

$E(\vec\phi(t))$ as defined in \eqnref{E} shares some similarities with the
Ising Hamiltonian.
Recall that the Ising Hamiltonian without self terms can be written as
\begin{equation}\eqnlabel{IsingHnoh}
	H = - \sum_{i,j,~i < j} J_{ij} s_i s_j  = - \frac{1}{2}\sum_{i,j,~i \neq j} J_{ij} s_i s_j.
\end{equation}

If we assume that every oscillator's phase settles to a binary value of either
$0$ or $\pi$\footnote{More generally, we use $\{2k\pi~|~k\in \mathbf{Z}\}$ and
$\{2k\pi+\pi~|~k\in \mathbf{Z}\}$ to represent the binary states.}, corresponding
to $s_i$ equal to $1$ or $-1$ in \eqnref{IsingH},
we have $\cos(\phi_i-\phi_j) = s_i \cdot s_j$.
Without loss of generality, we can assume $K = 1/2$.
In this case, the global Lyapunov function in \eqnref{E} matches
\eqnref{IsingHnoh} exactly --- the coupled oscillators are naturally minimising
the Ising Hamiltonian.

\begin{figure}[htbp!]
    \centering
    {
        \epsfig{file=figures/Kuramoto_with_without_SYNC.eps, width=0.9\linewidth}
    }
    \caption{Phases in the Kuramoto model \eqnref{Kuramoto} of 20 oscillators with random $\{J_{ij}\}$ generated by \texttt{rudy -rnd\_graph 20 50 10001}): \\ (a) without SYNC; (b) with $K_s = 1$. % encoding a random MAX-CUT problem generated by ...
    \figlabel{Kuramoto_with_without_SYNC}}
\end{figure}

However, only when the oscillator phases all settle to binary values is the
above reasoning valid.
A quick examination through simulation of \eqnref{Kuramoto} will show that this
is not the case in general, \eg, phases settle to analog values in
\figref{Kuramoto_with_without_SYNC} (a) with a random connection.
As discussed in \secref{intro}, one essential technique behind oscillator-based
Ising machines is the use of a second-order perturbation signal SYNC to make
oscillators behave like binary latches through the mechanism of SHIL.
As we show in \secref{theory}, the introduction of SYNC modifies the Kuramoto
model as follows.
\begin{equation}\eqnlabel{KuramotoSHIL}
	\frac{d}{dt} \phi_i(t) = - K\cdot \sum_{j=1,~j\neq i}^n J_{ij} \cdot \sin(\phi_i(t) - \phi_j(t))
						- K_s \cdot \sin(2\phi_i(t)),
\end{equation}

The new global Lyapunov function corresponding to \eqnref{KuramotoSHIL} can be
written as
\begin{equation}\eqnlabel{ESHIL1}
	E(\vec\phi(t)) = - K\cdot \sum_{i,j,~i\neq j} J_{ij} \cdot \cos(\phi_i(t) - \phi_j(t))
	  - \sum_{i=1}^n K_s \cdot \cos\left(2\phi_i(t)\right).
\end{equation}

When SYNC is strong enough, it enforces all phases $\phi_i$ to eventually take
values of either $0$ or $\pi$, as illustrated in
\figref{Kuramoto_with_without_SYNC} (b).
In this case, $\cos(2\phi_i) \approx 1$, and the Lyapunov function around these
steady states can be simplified as
\begin{equation}\eqnlabel{ESHIL2}
	E(\vec\phi(t)) \approx - K\cdot \sum_{i,j,~i\neq j} J_{ij} \cdot \cos(\phi_i(t) - \phi_j(t))
	  - n\cdot K_s,
\end{equation}
where $n\cdot K_s$ is a constant.
Therefore, the introduction of SYNC does not change the relative ``energy''
levels between valid binary phase configurations; it modifies them by the same
amount.
Instead of settling with continuous phases that minimises \eqnref{E}, the
system will now try to reach a binary state with the minimum Ising Hamiltonian.

Our analysis so far focuses on the deterministic model of oscillator-based
Ising machines.
Starting from a random initial condition, the coupled oscillator system follows
the gradient of $E(\vec\phi)$ to one of its local minima.
However, a physical realisation of the coupled oscillator network, especially
one that uses nanotechnology, will have intrinsic noise thus behave more
stochastically.
But this is not a disadvantage.
In the presence of noise, it becomes more likely for the coupled oscillators to
settle to the minima with lower $E$s; the probability of achieving better
solutions becomes higher.

The operation of oscillator-based Ising machines modelled in
\eqnref{KuramotoSDE} is controlled by several parameters --- the strength of
coupling $K$, the strength of SYNC $K_s$, and the noise level $K_n$.
Because of the Boltzmann law, we normally ramp up $K$ slowly in order to keep
the system at the thermodynamic equilibrium all the time.
$K_s$ can be kept constant, increased with time, or ramped up and down
repeatedly.
In fact, $K$, $K_s$, $K_n$ can all be time varying, creating various
annealing schedules.
As we show in \secref{examples}, this feature gives us much flexibility in the
operation of oscillator-based Ising machines for achieving good performance.



==> mechanism_old.tex <==
\section{Oscillator-based Ising Machines}\seclabel{mechanism}

\begin{equation}\eqnlabel{Kuramoto1}
	\frac{d}{dt} \phi_i(t) = \Delta\omega_i + \omega_0A_c\sum_j J_{ij} \cdot \sin(\phi_i(t) - \phi_j(t)),
\end{equation}

\begin{equation}\eqnlabel{Kuramoto2}
	\frac{d}{dt} \phi_i(t) = A_c\sum_j J_{ij} \cdot \sin(\phi_i(t) - \phi_j(t)).
\end{equation}

\begin{equation}\eqnlabel{Kuramoto3}
	\frac{d}{dt} \phi_i(t) = A_c\sum_j J_{ij} \cdot \sin(\phi_i(t) - \phi_j(t))
						- A_s \cdot \sin(2\phi_i(t)),
\end{equation}

The Kuramoto model is a gradient system \cite{smale1961gradient}. % find a better citation
There exists a global Lyapunov function for \eqnref{Kuramoto2}, which can be
considered as its ``energy'':
\begin{equation}\eqnlabel{E1}
	E(t) = A_c\sum_{i, j} J_{ij} \cdot \cos(\phi_i(t) - \phi_j(t)),
\end{equation}
such that
\begin{align}
	\frac{dE(t)}{dt} &= A_c\sum_{i} \left[ \frac{dE}{d\phi_i(t)} \cdot
                     \frac{d\phi_i(t)}{dt} \right] \\
				  &= A_c\sum_{i} \left[ - \left( \sum_{j} J_{ij} \cdot
					 \sin(\phi_i(t) - \phi_j(t))\right) \cdot \frac{d\phi_i(t)}{dt}
                     \right] \\
	              &= - \left|\left|\frac{d\vec \phi(t)}{dt}\right|\right|_2^2 \leq 0.
\end{align}

Therefore, the coupled oscillator system always attempts to minimize this
energy $E$.

$E$ as defined in \eqnref{E1} shares some similarities with the Ising Hamiltonian
in \eqnref{IsingH}.
If every oscillator's phase settles to a binary value of either $0$ or $\pi$,
corresponding to $s_i$ equal to $1$ or $-1$ in \eqnref{IsingH},
we have $\cos(\phi_i-\phi_j) = s_i \cdot s_j$.
Therefore, the coupled oscillators are naturally minimizing the Ising
Hamiltonian defined in \eqnref{IsingH}.
% In fact, this is also the mechanism with which many other
% coupled-oscillator-based computation schemes work for pattern recognition,
% image segmentation, \etc{}

This reasoning is only valid when we assume that the phases of all the
oscillators settle to binary values.
It is easy to prove that the assumption holds for two oscillators --- they will
settle with a phase difference of either $0$ or $\pi$ depending on the polarity
of coupling coefficient $J_{12}$.
But as the number of oscillators increases, the analysis quickly becomes
difficult and the phases can indeed settle to non-binary values.
In other words, the system becomes an analog computer like oscillator-based
associative memory arrays rather than a digital combinatorial optimizer.

As we discuss in \secref{intro}, one key technique behind oscillator-based
Ising machines is the use of a second-harmonic input SYNC to make oscillators
behave like binary latches through the mechanism of SHIL.
This modification changes the Kuramoto model to \eqnref{Kuramoto3} and results
in a new Lyapunov function as follows.

% \begin{align}
% 	E & = \sum_{i, j} \left[ J_{ij} \cdot \cos(\phi_i - \phi_j)
% 	  + \frac{K}{2} \cdot \cos\left(2\cdot (\phi_i - \phi_j)\right) \right] \\
% 	  & = \sum_{i, j} J_{ij} \cdot \cos(\phi_i - \phi_j)
% 	  + \frac{1}{2}n\cdot m\cdot K.
% \end{align}
\begin{equation}\eqnlabel{E2}
	E(t) = A_c\sum_{i, j} J_{ij} \cdot \cos(\phi_i(t) - \phi_j(t))
	  - \sum_{i} \frac{A_s}{2} \cdot \cos\left(2\cdot (\phi_i(t))\right).
\end{equation}

When SYNC is large enough, it enforces the phases $\phi_i$ to settle at either
$0$ or $\pi$, in which case the Lyapunov function can be simplified as
\begin{equation}\eqnlabel{E3}
	E(t) \approx A_c\sum_{i, j} J_{ij} \cdot \cos(\phi_i(t) - \phi_j(t))
	  - \frac{1}{2}(n+1)\cdot A_s,
\end{equation}
where $n+1$ is the total number of oscillators, with the last one being the
phase reference always representing logic 1.

Therefore, the introduction of SYNC does not change the relative ``energy''
levels between valid binary phase configurations; it modifies them by the same
amount.
It does not change the location of the ground state.
\ignore{

An oscillator with natural frequency $f_0$ can become injection locked when
perturbed by a small periodic external input at about the same frequency $f_1$
($f_1 \approx f_0$) --- the oscillator's frequency changes to $f_1$ and its
waveform locks onto the input with a constant phase difference.
% Because of injection locking, synchronization of coupled oscillators is an
% ubiquitous phenomenon in nature, \eg, metronomes on a same platform end up
% ticking in unison, fireflies synchronize their flashes, neurons fire in unison,
% \etc{}.
Sub-harmonic injection locking (SHIL) is a special type of injection locking.
When the external perturbation oscillates at integer multiples of the
oscillator's natural frequency, the oscillator's can develop multiple stable
responses that differ in the phase.
For example, when perturbed by a periodic input at $2f_1$, the oscillator will
lock to the input's sub-harmonic while developing bistable phase locks
separated by 180$^\circ$; in this paper, we call this perturbation a
synchronization signal (SYNC).
This bistable phase can be used to store a phase-based binary bit, making the
oscillator a logic latch.
It has been shown that such latches can be building blocks of oscillator-based
finite state machines for general-purpose Boolean computation
\cite{WaRoUCNC2014PHLOGON}.
% This mechanism is generic in almost all oscillators; the scheme is not specific
% to electrical ones.
% A broad choice of nonlinear oscillators --- from MEMS oscillators to optical
% lasers, from spin-torque nano-oscillators (STNOs) to oscillating biochemical
% reactions and neurons --- become potential candidates for Boolean computation
% systems.

If we lower SYNC and reduce the effect of SHIL, due to intrinsic phase noise
and detuning, the oscillator will have phase response that stochastically flips
between the bistable states --- it becomes a binary random number generator.
If two of these oscillators are coupled, \eg, through resistive connection,
instead of having four states \{00\}, \{01\}, \{10\}, \{11\} with even
probabilities, they will have higher probability to end up in \{00\} and \{11\}
--- these two states become the ground states of this simple size-2 Ising
model.
More complicated Ising Hamiltonians can be encoded by coupling more
oscillators, in a similar way to the existing Ising machine proposals.
Specifically, a larger coefficient $J_{ij}$ in \eqnref{IsingH} is represented
with a larger conductance in the coupling.

To study this mechanism more properly, we start from the phase macromodel of a
single nonlinear self-sustaining oscillator.
Such an oscillator under perturbation can be described mathematically as a set
of Differential Algebraic Equations (DAEs):
\begin{equation}\eqnlabel{DAE}
	\frac{d}{dt} \vec q(\vec x) + \vec f(\vec x)  + \vec b(t) = \vec 0
\end{equation}
where $\vec x \in \mathbf{R}^n$ are the unknowns in the system, 
$\vec b(t)$ is a small time-varying input.
The oscillator's response can be approximated well as
\begin{equation}\eqnlabel{xt}
	\vec x(t) = \vec x_s(t + \alpha(t))
\end{equation}
where $x_s(t)$ is the oscillator's steady state response without perturbation
($\vec b(t) \equiv \vec 0$);
$\alpha(t)$ is the phase shift caused by the external input and is governed by
the following differential equation:
\begin{equation}\eqnlabel{PPV}
	\frac{d}{dt} \alpha(t) = \vec v^T(t + \alpha(t)) \cdot \vec b(t)
\end{equation}
where the vector $\vec v(t)$ is known as the Perturbation Projection Vector
(PPV) \cite{DeMeRoTCAS2000} of the oscillator.
Assume the oscillator's natural frequency is
$\omega_0 = 2\pi f_0 = 2\pi/T_0$.
Then $\vec v(t)$ is a $T_0$-periodic vector that can be extracted
numerically from the DAEs of the oscillator without knowing any information
about the input $\vec b(t)$.
Put in other words, it is a property intrinsic to the oscillator that 
captures its phase response to small external inputs.
PPV can be used to model and predict injection locking effectively
\cite{LaRoMTT2004}.

When the external perturbation $\vec u(t)$ is periodic itself with frequency
$\omega_1 = 2\pi f_1 = 2\pi /T_1$, equation \eqnref{PPV} can be rewritten as
\begin{equation}\eqnlabel{PPVphiOLDTWO}
\frac{d}{dt} \Delta \phi(t) = \omega_0-\omega_1 + \omega_0 \cdot \vec v_{(2\pi)}^T(\omega_1\cdot t +
\Delta \phi(t)) \cdot \vec u_{(2\pi)}(\omega_1\cdot t),
\end{equation}
where $\Delta \phi(t) = (\omega_0-\omega_1)\cdot t + \omega_0\cdot \alpha(t)$
--- when injection locking occurs, it is the phase difference between the
oscillator's response and the periodic perturbation;
both $\vec v_{(2\pi)}$ and $\vec u_{(2\pi)}$ are $2\pi$-periodic functions ---
$\vec v_{(2\pi)}(t) = \vec v(t/\omega_0)$,
$\vec u_{(2\pi)}(t) = \vec u(t/\omega_1)$.

In a special case, when both $\vec v(t)$ and $\vec u(t)$ are sinusoidal scaler
functions, \ie, we assume $\vec v_{(2\pi)}(t) = A_v\sin(t)$
and $\vec u_{(2\pi)}(t) = A_u\cos(t + \Delta \phi_u)$,
\eqnref{PPVphi} can be rewritten as 
{\small
\begin{align}
\frac{d}{dt} \Delta \phi(t)
=& \omega_0-\omega_1+\omega_0 \cdot
A_v\sin\left(\omega_1 t + \Delta \phi(t)\right)
\cdot
A_u\cos\left(\omega_1 t + \Delta \phi_u\right)\\
=& \omega_0-\omega_1+\omega_0 \cdot [
\frac{1}{2}A_vA_u\sin\left(\Delta \phi(t) - \Delta \phi_u\right) \nonumber\\
&+
\frac{1}{2}A_vA_u\sin\left(2\omega_1 t + \Delta \phi(t) + \Delta \phi_u\right)
].
\end{align}
}

The last term is fast varying with time. If we average it out and let
$A_1=\frac{1}{2}A_vA_u$, we get
\begin{equation}\eqnlabel{Adler}
    \frac{d}{dt} \Delta \phi(t) =
    \omega_0-\omega_1+\omega_0 A_1 \sin\left(\Delta \phi(t) - \Delta \phi_u\right).
\end{equation}

\eqnref{Adler} is known as the Adler's equation \cite{Adler1973}.
It can explain many interesting properties of injection locking.
For example, if we assume there to be no detuning, \ie, $\omega_0=\omega_1$,
the steady state equation $\frac{d}{dt} \Delta \phi(t) = 0$ has two sets of
solutions --- $\phi_u + 2k\pi$ and $\phi_u + 2k\pi + \pi$,
where $k\in \mathrm{Z}$.
We can linearize the system around the solutions and analyze the slopes, which
indicate the stability of these solutions.
Results show that the latter sets are stable.
This indicates that the oscillator's phase will be stably locked to the input
with only one possible phase shift value under injection locking, which matches
observation.
Moreover, when there is detuning, \ie, $\omega_0 \ne \omega_1$, Adler's
equation can also be used to estimate the locking range.

If we further assume that the waveform of each oscillator is also sinusoidal,
we can derive the Kuramoto model for coupled oscillators
\cite{acebron2005kuramoto} from the Adler's equation:
\begin{equation}\eqnlabel{Kuramoto1}
	\frac{d}{dt} \phi_i(t) = \Delta\omega_i + \omega_0A_c\sum_j J_{ij} \cdot \sin(\phi_i(t) - \phi_j(t)),
\end{equation}
where $\phi_i(t)$ is the phase of the $i$\textsuperscript{th} oscillator in the
system; $\omega_0$ is the frequency of the synchronized coupled oscillator
system; $\Delta\omega_i$ is the phase difference between each oscillator's
natural frequency and $\omega_0$; $A_c$ is a scalar representing the coupling
strength.

If we assume no frequency variation in all the oscillators for the moment, \ie,
$\Delta\omega_i=0$, and normalize $\omega_0$ to $1$, we can simplify
\eqnref{Kuramoto1} as
\begin{equation}\eqnlabel{Kuramoto2}
	\frac{d}{dt} \phi_i(t) = A_c\sum_j J_{ij} \cdot \sin(\phi_i(t) - \phi_j(t)).
\end{equation}

Similar analysis can be applied when we include SHIL in the system.
For a single oscillator, when its input has a periodic entry at $2\omega_1$, we
assume that the corresponding entry in $\vec v(t)$ also has a second harmonic
at $2\omega_0$, \ie, $\vec v_{(2\pi)}(t) = A_{v2}\sin(2t)$ and $\vec
u_{(2\pi)}(t) = A_{u2}\cos(2t + \Delta \phi_u)$,
Then following the same procedures as above, we get
\begin{equation}\eqnlabel{Adler2}
\frac{d}{dt} \Delta \phi(t) = \omega_0-\omega_1+\omega_0 A_2 \sin\left(2\Delta \phi(t) - \Delta \phi_u)\right),
\end{equation}
where $A_2=\frac{1}{2}A_{v2}A_{u2}$.
Steady state analysis of \eqnref{Adler2} indicates that the oscillator can lock
to the input with two stable phases, separated by $\pi$.

Incorporating \eqnref{Adler2} into the Kuramoto model \eqnref{Kuramoto2},
assuming that each oscillator is receiving an identical second-harmonic
periodic input SYNC, we can write the new coupled oscillator system equation as
% \begin{equation}
% 	\frac{d}{dt} \phi_i = \sum_j \left[J_{ij} \cdot \sin(\phi_i - \phi_j)
% 						+ K \cdot \sin\left(2\cdot (\phi_i)\right)\right].
% \end{equation}
\begin{equation}\eqnlabel{Kuramoto3}
	\frac{d}{dt} \phi_i(t) = A_c\sum_j J_{ij} \cdot \sin(\phi_i(t) - \phi_j(t))
						- A_s \cdot \sin(2\phi_i(t)),
\end{equation}
where scaler $A_s$ models the coupling strength from SYNC.

Note that the assumptions of sinusoidal PPV and sinusoidal waveforms are not
necessary.
Generalized Adler's Equation (GAE) \cite{BhRoASPDAC2009} has been developed for
handling arbitrary PPV shapes, and it provides good approximations to the
injection-locked solutions of \eqnref{PPVphi}.
This indicates that there are also generalized Kuramoto models where the $\sin()$
function can be replaced with arbitrary periodic functions, and oscillators can
be engineered to have the desired properties.

The Kuramoto model is a gradient system \cite{smale1961gradient}. % find a better citation
There exists a global Lyapunov function for \eqnref{Kuramoto2}, which can be
considered as its ``energy'':
\begin{equation}\eqnlabel{E1}
	E(t) = A_c\sum_{i, j} J_{ij} \cdot \cos(\phi_i(t) - \phi_j(t)),
\end{equation}
such that
\begin{align}
	\frac{dE(t)}{dt} &= A_c\sum_{i} \left[ \frac{dE}{d\phi_i(t)} \cdot
                     \frac{d\phi_i(t)}{dt} \right] \\
				  &= A_c\sum_{i} \left[ - \left( \sum_{j} J_{ij} \cdot
					 \sin(\phi_i(t) - \phi_j(t))\right) \cdot \frac{d\phi_i(t)}{dt}
                     \right] \\
	              &= - \left|\left|\frac{d\vec \phi(t)}{dt}\right|\right|_2^2 \leq 0.
\end{align}

Therefore, the coupled oscillator system always attempts to minimize this
energy $E$.

$E$ as defined in \eqnref{E1} shares some similarities with the Ising Hamiltonian
in \eqnref{IsingH}.
If every oscillator's phase settles to a binary value of either $0$ or $\pi$,
corresponding to $s_i$ equal to $1$ or $-1$ in \eqnref{IsingH},
we have $\cos(\phi_i-\phi_j) = s_i \cdot s_j$.
Therefore, the coupled oscillators are naturally minimizing the Ising
Hamiltonian defined in \eqnref{IsingH}.
% In fact, this is also the mechanism with which many other
% coupled-oscillator-based computation schemes work for pattern recognition,
% image segmentation, \etc{}

This reasoning is only valid when we assume that the phases of all the
oscillators settle to binary values.
It is easy to prove that the assumption holds for two oscillators --- they will
settle with a phase difference of either $0$ or $\pi$ depending on the polarity
of coupling coefficient $J_{12}$.
But as the number of oscillators increases, the analysis quickly becomes
difficult and the phases can indeed settle to non-binary values.
In other words, the system becomes an analog computer like oscillator-based
associative memory arrays rather than a digital combinatorial optimizer.

As we discuss in \secref{intro}, one key technique behind oscillator-based
Ising machines is the use of a second-harmonic input SYNC to make oscillators
behave like binary latches through the mechanism of SHIL.
This modification changes the Kuramoto model to \eqnref{Kuramoto3} and results
in a new Lyapunov function as follows.

% \begin{align}
% 	E & = \sum_{i, j} \left[ J_{ij} \cdot \cos(\phi_i - \phi_j)
% 	  + \frac{K}{2} \cdot \cos\left(2\cdot (\phi_i - \phi_j)\right) \right] \\
% 	  & = \sum_{i, j} J_{ij} \cdot \cos(\phi_i - \phi_j)
% 	  + \frac{1}{2}n\cdot m\cdot K.
% \end{align}
\begin{equation}\eqnlabel{E2}
	E(t) = A_c\sum_{i, j} J_{ij} \cdot \cos(\phi_i(t) - \phi_j(t))
	  - \sum_{i} \frac{A_s}{2} \cdot \cos\left(2\cdot (\phi_i(t))\right).
\end{equation}

When SYNC is large enough, it enforces the phases $\phi_i$ to settle at either
$0$ or $\pi$, in which case the Lyapunov function can be simplified as
\begin{equation}\eqnlabel{E3}
	E(t) \approx A_c\sum_{i, j} J_{ij} \cdot \cos(\phi_i(t) - \phi_j(t))
	  - \frac{1}{2}(n+1)\cdot A_s,
\end{equation}
where $n+1$ is the total number of oscillators, with the last one being the
phase reference always representing logic 1.

Therefore, the introduction of SYNC does not change the relative ``energy''
levels between valid binary phase configurations; it modifies them by the same
amount.
It does not change the location of the ground state.
}

\ignore{
	Steady states of such a coupled oscillator network can be reached by
	several types of ``annealing'' --- decreasing noise, increasing coupling, and
	pumping up SYNC.
	It is provable that every steady state corresponds to a local optimum of the
	Ising Hamiltonian.
	In the presence of noise, with sufficient annealing time, the network will tend
	to settle to the most stable state, corresponding to the ground state of Ising
	Hamiltonian, \aka{} the global optimum of the combinatorial problem.

	SHIL makes almost any oscillator work as a logic latch that can store one bit
	of information; storing this bit securely enables oscillator-based Boolean
	computation. An oscillator latch is also very useful even when the bit is not
	entirely secure. Due to phase noise and detuning in the oscillator, the
	phase-based bit stored in the latch is a random process --- it flips from now
	and then. Everytime it is measured, it can randomly assume 0 or 1 value. An
	oscillator becomes a binary random number generator. Given today's oscillator
	technology, they can be very compact compared with existing solutions.

	Moreover, the probability of this random variable at a given time can be
	controlled through coupling between oscillator latches. For example, if there
	are two oscillators under weak SHIL, their phase values can represent {0, 0},
	... {1, 1} (four sets of values). If they are connected through a resistor (in
	electrical domain), such that the phase of one of them affects the other. As is
	obvious to see, if the coupling is strong enough, I.e., the resistor is very
	small such that the two oscillators are connected to each other through a short
	connection, their phases can only settle to {0,0} and {1,1} values. Similarly,
	when the coupling is chosen appropriately, {0,1} and {1,0} may still have some
	probability, but much lower than those of the other "ground states". If we let
	this two oscillator system settle to the steady state, their phases will have
	solved an optimization problem (or a logic problem) whose solutions require that
	the two values are the same. More complex problems can be represented and
	solved with more complicated coupling between the oscillator latches.

	Recently, Ising machines have been proposed for invertible logic computation
	applications, such as factorization. The idea is similar. If the logic problem
	is formulated as an optimization problem such that the ground states correspond
	to its valid solutions, when the Ising model settle to its ground state, the
	solutions solve the logic problem. In this way, a connection for addition can
	also be used to solve for subtraction; multipliers can be used for
	factorization.

	Compared with the existing ideas on the practical implementation of Ising
	machines, our idea of oscillator-based Ising machine has several advantages
	(features). Firstly, the oscillator technology is ready available, and general
	across many fields of engineering. The idea can be demonstrated (or
	experimented with) using well-developed CMOS oscillators. It can also be
	implemented with novel oscillator devices, such as spin torque, MEMS,
	memristor-based ones. Many of them are nano-scale and energy efficient. Many
	are also large-scale integrable  on chip already. Note that on-chip Ising
	machine has been proposed and implemented before, with standard CMOS
	level-based latches. But applications such as general combinatorial
	optimization or invertible logic have not been achieved; the only demonstration
	was pattern recognition, the standard task suitable for hopfield network (which
	is deterministic, no need to control noise, easy to control coupling).

	Oscillator-based Ising machines normally require sparse connections between
	vertices. This is rarely a problem since most real world problems can be
	formulated into sparse coupling [], or even into a grid of nodes [] if
	auxiliary nodes are introduced.
	Recent work [] use FPGA to form virtual connections, in order to achieve full
	connection among vertices.
	The same idea still applies to oscillator-based Ising machines if desired.

	We shall not confuse oscillator-based Ising machines with quantum annealers,
	such as those being developed at D-Wave [].
	No quantum annealing is available.
	The performance will be worse for larger-scale problems.
	But since oscillators are easily integrable and they mostly work at room
	temperature, they are cost and energy efficient, and can scale faster and more
	easily.
	Also, more auxiliary vertices normally result in better convergence to the
	ground state of the original optimization problem. 
}

\ignore{
One major obstacle to the practical implementation of large-scale Ising
machines is variability.
Researchers of SRAM-based CMOS Ising machines explicitly attribute the
``limited efficacy'' to the variations in SRAMs \cite{yamaoka2016IsingCMOS}.
Indeed, SRAMs are not good random number generators --- process variations
often give them preferences of generating either 1s or 0s.
Ising machines based on nano-magnets \cite{camsari2017pbits} are likely to
suffer from the same problem in hardware implementations.
Specifically, each nano-magnet will prefer either the ``up'' or ``down'' state
after fabrication, the effects of which are yet to be studied.
In comparison, the binary states in an oscillator are defined based on
phase/timing, and are thus perfectly ``symmetric'' --- there is no mechanism
making an oscillator prefer phase 0 to phase $\pi$ under SHIL.
This symmetry can lead to markedly improved performances over the SRAM-based
scheme in large-scale implementations.

Even so, there are still variations in coupled oscillators, coming from another
source --- the variability of the oscillators' natural frequencies.
Taking this into consideration, we rewrite the Kuramoto model in
\eqnref{Kuramoto3} as
% \begin{equation}
% 	\frac{d}{dt} \phi_i = \omega_i
% 	                    + \sum_j \left[J_{ij} \cdot \sin(\phi_i - \phi_j)
% 						+ K \cdot \sin\left(2\cdot (\phi_i -
%                           \phi_j)\right)\right].
% \end{equation}
% 
% \begin{equation}
% 	E = \sum_{i} \omega_{i} \cdot \phi_i
% 	    + \sum_{i, j} J_{ij} \cdot \cos(\phi_i - \phi_j)
% 	    + \frac{1}{2}n\cdot m\cdot K.
% \end{equation}
\begin{equation}\eqnlabel{Kuramoto_var}
	\frac{d}{dt} \phi_i(t) = \Delta\omega_i
	                    + A_c\sum_j J_{ij} \cdot \sin(\phi_i(t) - \phi_j(t))
						- A_s \cdot \sin\left(2\phi_i(t)\right).
\end{equation}

And the corresponding Lyapunov function becomes
\begin{equation}\eqnlabel{E4}
	E(t) = \sum_{i} \Delta\omega_{i} \cdot \phi_i(t)
	    + A_c\sum_{i, j} J_{ij} \cdot \cos(\phi_i(t) - \phi_j(t))
	    - \frac{1}{2}(n+1)\cdot A_s.
\end{equation}

Note that \eqnref{E4} differs from \eqnref{E3} only by a weighted sum of
$\phi_i$ --- it represents essentially the same ``energy'' landscape but tilted
linearly with the optimization variables.
While it can still change the locations and values of solutions, its effects
are easy to analyze given a specific combinatorial optimization problem.
Also, as the coupling coefficient $A_c$ gets larger, the effect of detuning is
reduced.

The OPO-based Ising machine also uses phase-based logic encoding
\cite{marandi2014network}, but it does not use self-sustaining oscillators.
The variations in frequency and amplitude are minimized by generating the
pulses from the same laser and letting them travel through the same optical
fiber.
As such, the implementation is not easy to miniaturize.
One way towards integration is to use individual ring resonators as parametric
oscillators.
Then process variations in integrated photonics will create problems again.
And analyzing variation's effects on parametric oscillators appears to be an
unsolved problem; it is much more difficult than the analysis above for coupled
oscillators.

Our analysis so far focuses only on the deterministic model of oscillator-based
Ising machines, thus is not complete.
Starting from a random initial condition, coupled oscillators evolve in a
deterministic manner, in an effort to minimize the global Lyapunov function $E$
in \eqnref{E3}, which corresponds to the Ising Hamiltonian in \eqnref{IsingH}.
This is a dynamical-system-based implementation of the gradient descent
algorithm that can find local minima of a function.
Therefore, like gradient descent, its effectiveness in finding the global
minimum is limited.
However, we can reasonably suspect that, if there is noise in the system, it
becomes more likely for the coupled oscillators to settle to the minima with
lower $E$s; like simulated annealing, the probability of achieving the ground
state becomes higher.

To analyze this hypothesis, we first introduce noise into the coupled
oscillator model.
One common way is to assume there is white noise in the central frequencies,
which can be modelled as additive white noise in the Kuramoto model.
\begin{equation}\eqnlabel{noise1}
	\frac{d}{dt} \phi_i(t) = A_c\sum_j J_{ij} \cdot \sin(\phi_i(t) - \phi_j(t))
						- A_s \cdot \sin(2\phi_i(t)) + A_n\xi_i(t),
\end{equation}
where $\xi_i(t)$ represents Gaussian white noise with zero mean and
correlator $\langle\xi_i(t),~\xi_i(\tau)\rangle = \delta(t-\tau)$;
scaler $A_n$ represents the magnitude of noise.

\eqnref{noise1} can be rewritten as a stochastic differential equation (SDE).
\begin{equation}\eqnlabel{noise2}
	d\phi_{it} = \left[A_c\sum_j J_{ij} \cdot \sin(\phi_{it} - \phi_{jt})
						- A_s \cdot \sin(2\phi_{it}) \right]dt + A_ndW_t.
\end{equation}

From it, one can derive master equations describing the time evolution of the
probability of the system to occupy each state.
Since we are mainly interested in the steady state, here we can directly apply
the Boltzmann law from statistical mechanics \cite{landau1969statistical}.
For a system with discrete states $\vec s_i$, $i=1,\cdots,M$, if each state is
associated with an energy $E_i$, the probability $P_i$ for the system to be at
each state can be written as follows.
\begin{equation}
	P_i = {\frac{e^{- E_i / k T}}{\sum_{j=1}^{M}{e^{- E_j / k T}}}},
\end{equation}
where $k$ is the Boltzmann constant, $T$ is the thermodynamic temperature of
the system.
While $k$ and $T$ are concepts specific to statistical mechanics, in this
context the product $kT$ correlates with the magnitude of $A_n$.

Given two spin configurations $\vec s_1$ and $\vec s_2$, the ratio between
their probabilities is known as the Boltzmann factor:
\begin{equation}
\frac{P_2}{P_1} = e^{\frac{E_1 - E_2}{kT}}.
\end{equation}

In oscillator-based Ising machines, the energy at a spin configuration is
\begin{align}
	E(\vec s) &= A_c\sum_{i, j} J_{ij} s_is_j - \frac{1}{2}(n+1)\cdot A_s \\
	     &= A_c\sum_{i, j} J_{ij} s_is_j - Const, \eqnlabel{E5}
\end{align}

Therefore,
\begin{equation}
E_1 - E_2 \propto A_c.
\end{equation}

If $\vec s_1$ is the higher energy state, \ie, $E_1 > E_2$, as the coupling
strength $A_c$ increases, it becomes less and less likely for the system to
stay at $\vec s_1$. The system prefers the lowest energy state in the presence
of noise.

Note that the Boltzmann law describes systems with states that have physical
energies.
A coupled oscillator system, like many computational systems, its dissipative
in its nature, \ie, it is a thermodynamically open system operating far from
equilibrium.
As such, it does not have a physical energy associated with its states.
However, it is provable that a global Lyapunov function, if it exists, can be
used as an energy function to derive the same Boltzmann law
\cite{yuan2010lyapunov}.
Therefore, the above reasoning for achieving better minima under noise still
holds for oscillator-based Ising machines.

The operation of oscillator-based Ising machines modelled in \eqnref{noise1} is
controlled by several parameters --- the mutual coupling strength $A_c$, the
SYNC coupling strength $A_s$, and the noise level $A_n$.
Because of the Boltzmann law, we normally ramp up $A_c$ slowly in order to keep
the system at the thermodynamic equilibrium all the time.
$A_s$ can be kept constant or ramped up in the meanwhile.
In fact, $A_c$, $A_s$, $A_n$ can all be time varying, resulting in various
annealing profiles.
As we show in \secref{examples}, this property gives us much flexibility in the
engineering of oscillator-based Ising machines.

} % ignore


\section{From Oscillator's Phase Macromodels to the Ising Hamiltonian}\seclabel{theory}

In this section, we present the theory behind the operation of oscillator-based
Ising machines, starting with modelling the phase response of an oscillator
under perturbation.

A single nonlinear self-sustaining oscillator is an autonomous dynamical system,
usually modelled using Differential Algebraic Equations (DAEs) in the following
form.
\begin{equation}\eqnlabel{DAEnoB}
	\frac{d}{dt} \vec q(\vec x(t)) + \vec f(\vec x(t))  = \vec 0,
\end{equation}
where $\vec x(t) \in \mathbf{R}^n$ represents the unknowns in the system;
$\vec q(.)$ and $\vec f(.)$ are $\colon \mathbf{R}^n \to \mathbf{R}^n$ functions,
representing the differential and algebraic parts of the DAE respectively.

A self-sustaining oscillator has a nonconstant $T_0$-periodic solution $\vec
x^*_s(t)$ to \eqnref{DAEnoB}, satisfying $\vec x^*_s(t+T_0) = \vec x^*_s(t)$.

When this oscillator is under a time-varying perturbation modelled as $\vec
b(t) \in \mathbf{R}^n$, its DAE can be written as follows.
\begin{equation}\eqnlabel{DAE}
	\frac{d}{dt} \vec q(\vec x(t)) + \vec f(\vec x(t))  + \vec b(t) = \vec 0.
\end{equation}

If the perturbation is small, the oscillator's perturbed response can be
approximated well as
\begin{equation}\eqnlabel{xt}
	\vec x^*(t) = \vec x^*_s(t + \alpha(t)),
\end{equation}
where $\alpha(t)$ is the phase shift caused by the external input and is
governed by the following differential equation:
\begin{equation}\eqnlabel{PPV}
	\frac{d}{dt} \alpha(t) = \vec p^T(t + \alpha(t)) \cdot \vec b(t)
\end{equation}
where the time-varying vector $\vec p(t)$ is known as the Perturbation
Projection Vector (PPV) \cite{DeMeRoTCAS2000} of the oscillator.
It is $T_0$-periodic, and is a property intrinsic to the oscillator that
captures its phase response to small external inputs.
$\vec p(t)$ and can be calculated analytically [] or numerically [][] from the
oscillator's DAE without knowing any information about the input $\vec b(t)$.
% It can be used to model and predict injection locking effectively \cite{LaRoMTT2004} [].

When the external input $\vec b(t)$ is a periodic signal with frequency
$\omega^* = 2\pi f^* = 2\pi /T^*$ and phase perturbation $\phi_{in}(t)$,
equation \eqnref{PPV} can be rewritten as
\begin{equation}\eqnlabel{PPVphiOLD}
\frac{d}{dt} \phi(t) = \omega_0-\omega^* + \omega_0 \cdot \vec p_{(2\pi)}^T(\omega^*\cdot t +
\phi(t)) \cdot \vec b_{(2\pi)}(\omega^*\cdot t + \phi_{in}(t)),
\end{equation}
where $\phi(t) = (\omega_0-\omega^*)\cdot t + \omega_0\cdot \alpha(t)$
--- when injection locking occurs, it is the difference between the phase of
oscillator's response and that of the periodic perturbation;
both $\vec v_{(2\pi)}$ and $\vec b_{(2\pi)}$ are $2\pi$-periodic functions ---
$\vec p_{(2\pi)}(t) = \vec p(t/\omega_0)$,
$\vec b_{(2\pi)}(t) = \vec b(t/\omega^*)$.

Use MPDE (Multi-time Partial Differetial Equation), slow time $t_1$, fast time $t_2$.

\begin{align}\eqnlabel{PPVphiMPDE}
\frac{\partial \hat\phi(t_1,~t_2)}{\partial t_1} + \frac{\partial \hat\phi(t_1,~t_2)}{\partial t_2}
= & ~\omega_0-\omega^* \nonumber\\
& + \omega_0 \cdot \vec p_{(2\pi)}^T(\omega^*\cdot t_2 +
\hat\phi(t_1)) \cdot \vec b_{(2\pi)}(\omega^*\cdot t_2 + \phi_{in}(t_1)),
\end{align}

Because $\hat\phi(t,~t) = \phi(t)$, we can solve for PDE $\hat\phi(.,~.)$ instead.

The solution is fast varying in $t_2$ dimension. So we average along the $t_2$
dimension --- replacing the $t_2$-varying solution with a constant for every $t_1$.
Note that the assumption is valid when the phase of oscillation is changing
much more slowly than the oscillation itself.
In this case, we approximate $\hat\phi(t_1,~t_2) \approx \bar\phi(t_1) \equiv \phi(t_1)$.

\begin{align}\eqnlabel{PPVphiMPDEt1}
\frac{d \bar\phi(t_1)}{d t_1}
= & ~\omega_0-\omega^* \nonumber\\
& + \omega_0 \cdot \int_0^{2\pi} \vec p_{(2\pi)}^T(\omega^*\cdot t_2 +
\bar\phi(t_1)) \cdot \vec b_{(2\pi)}(\omega^*\cdot t_2 + \phi_{in}(t_1)) ~ d t_2 \\
= & ~\omega_0-\omega^* \nonumber\\
& + \omega_0 \cdot \int_0^{2\pi} \vec p_{(2\pi)}^T(\omega^*\cdot t_2 +
\bar\phi(t_1) -  \phi_{in}(t_1)) \cdot \vec b_{(2\pi)}(\omega^*\cdot t_2) ~ d t_2.
\end{align}

Define
\begin{equation}
c(t) = \int_0^{2\pi} \vec p_{(2\pi)}^T(t + \tau) \cdot \vec b_{(2\pi)}(\tau) ~ d \tau.
\end{equation}

$c(t)$ is a $2\pi$-periodic function.
It is the cross-correlation of the two functions $\vec p_{(2\pi)}(.)$ and $\vec b_{(2\pi)}(.)$.

\begin{equation}
\frac{d}{d t} \phi(t) = ~\omega_0-\omega^* + \omega_0 \cdot c(\phi(t) -  \phi_{in}(t))
\end{equation}

Special case. For LC oscillators with resistive coupling to the node with $A\cdot \sin(t)$ waveform,
$\vec p_{(2\pi)}(.)$ is proportional to $\cos(t)$, making $c(\phi(t) -  \phi_{in}(t))$ proportional to 
$\sin(\phi(t) -  \phi_{in}(t))$.
Then we have the Adler's equation.

\begin{equation}
\frac{d}{d t} \phi(t) = ~\omega_0-\omega^* + \omega_0 \cdot \sin(\phi(t) -  \phi_{in}(t)).
\end{equation}

Another special case, when $\vec b(t)$ is second harmonic perturbation, \ie, it is $\pi$-periodic.


For the $i$th oscillator in a coupled oscillator network,
\begin{align}
\frac{d}{dt} \phi_i(t) = & ~\omega_i-\omega^* + \omega_i \cdot \sum_{j=1,~j\neq i}^n \left[J_{ij} \cdot \vec p_{ij}^T(\omega^*\cdot t +
\phi_i(t)) \cdot \vec b_j(\omega^*\cdot t + \phi_{j}(t))\right] \nonumber\\
& + \omega_i \cdot h_i \cdot \vec p_i^T(\omega^*\cdot t + \phi_i(t)) \cdot \vec b_0(\omega^*\cdot t)
\end{align}
where $\omega_i$ is the frequency of this oscillator,
$\omega^*$ is the central frequency for the couple oscillators,
$\vec p_{ij}(.)$ is the $2\pi$-periodic PPV of the $i$th oscillator, with perturbation from the $j$th oscillator,
$\vec b_j(.)$ is the $2\pi$-periodic perturbation from the $j$th oscillator.

$\vec p_i(.)$ is the $2\pi$-periodic PPV of the $i$th oscillator, with perturbation from a reference signal,
$\vec b_0(.)$ is the $2\pi$-periodic reference signal.

\begin{align}
\frac{d}{d t} \phi_i(t) =& ~\omega_i-\omega^* + \omega_i \cdot
\sum_{j=1,~j\neq i}^n \left[ J_{ij} \cdot c_{ij}(\phi_i(t) -  \phi_j(t)) \right]
\nonumber\\
& + \omega_i \cdot h_i \cdot \vec d_i(\phi_i(t))
\end{align}

\begin{align}
c_{ij}(t) =& \int_0^{2\pi} \vec p_{ij}^T(t + \tau) \cdot \vec b_j(\tau) ~ d \tau.\\
d_i(t) =& \int_0^{2\pi} \vec p_i^T(t + \tau) \cdot \vec b_0(\tau) ~ d \tau.
\end{align}

\begin{align}
C_{ij}(t) =& \int_0^{t} c_{ij}(\tau) ~ d \tau + C_{0ij}.\\
D_{i}(t) =& \int_0^{t} d_{i}(\tau) ~ d \tau + D_{0i}.
\end{align}
$C_{0ij}$ and $D_{0i}$ are arbitrary constants.

\begin{equation}
	E(t) = A_c\sum_{i, j} J_{ij} \cdot \cos(\phi_i(t) - \phi_j(t)),
\end{equation}


==> newcommands-eg-ie-etc.tex <==
% eg, ie, etc, wrt, viz newcommands
\newcommand{\eg}{{\it e.g.\@}} % \@ for normal spacing after. use: \eg\/ or \eg,
\newcommand{\ie}{{\it i.e.\@}} 
\newcommand{\wrt}{{\it wrt}}
\newcommand{\viz}{{\it viz.\@}}
\newcommand{\vs}{{\it vs.\@}}
\newcommand{\aka}{{\it aka}}
\newcommand{\apriori}{{\it a priori}}
\newcommand{\etc}{\textit{etc.\@}}                                                
% etc defined so that there is only a single period after it if it is followed 
% by a period
% see: http://en.wikibooks.org/wiki/TeX/def                                      
% see: http://www.tug.org/pipermail/texhax/2004-July/002449.html                 
% see: http://en.wikibooks.org/wiki/TeX/if                                       
%\ifx \etc \undefined                                                             
%  %\def\myarg{#1}                                                                
%  %\def\myfullstop{.}                                                            
%  %\def\etc{#1}{\textit{etc} arg is ``\myarg'' \ifx\myarg\myfullstop\then.\else.#1\fi\/}
%  \def\etc#1{\textit{etc}\if#1..\else.#1\fi}                                     
%\fi                                                                              
%                        


==> newcommands-for-bibtex.tex <==
\newcommand{\BP}{({\textbf{Best Paper}})} % used in bibliography
\newcommand{\BPnom}{({\textbf{Best Paper Nomination}})} % used in bibliography
\newcommand{\IP}{({\textbf{Invited}})} % used in bibliography
\newcommand{\presenter}[1]{#1} % used in bibliography
\newcommand{\putDOI}[1]{#1}
%\newcommand{\putDOI}[1]{}
\newcommand{\DP}{\textbf{(Distinguished Paper)}}


==> newcommands-highlight-ignore-comments-annotations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% newcommands for ignoring, commenting, annotating, highlighting
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ignore}[1]{}
\let\IGNORE=\ignore
%\newcommand{\comment}[1]{} % conflicts with something predefined
\newcommand{\COMMENT}[1]{}
\newcommand{\jrcomment}[1]{{\color{blue}#1}}
\newcommand{\agcomment}[1]{{\color{mydarkgreen}#1}}
\let\agc=\agcomment
\let\jc=\jrcomment
\newcommand{\redHL}[1]{{\color{red}\bf #1}}
\newcommand{\REDHL}[1]{{\color{red}\bf #1}}
\newcommand{\blueHL}[1]{\textbf{\color{blue}#1}}
\newcommand{\jsugg}[1]{\textit{\color{blue}#1}}
\newcommand{\jpvt}[1]{\textit{\color{red}#1}}
%\newcommand{\jsumm}[1]{{\color{blue}{{\uline{\textit{#1}}}}}}
\newcommand{\jsumm}[1]{\centerline{\color{blue}{{\uline{\textit{#1}}}}\\}}
\newcommand{\jkill}[1]{{\color{blue}\sout{#1}}}
\newcommand{\toputback}[1]{{\blueHL{PUT THIS BACK:} #1}}
\newcommand{\jemph}[1]{\textbf{\uline{#1}}}
\newcommand{\jques}[1]{{\color{blue}#1?}}
\let\jnoteignored=\ignore
	
%\newcommand{\jnote}[1]{\textit{\color{blue}#1}}
%\newcommand{\jnote}[1]{\centerline{\color{mydarkgreen}{{\uline{\textit{#1}}}}\\}}
\newcommand{\jnote}[1]{{\color{mydarkgreen}\textit{\uline{#1}}}}
\ignore{
    \newcommand{\jnote}[1]{% using fixme
    	\renewcommand{\fxnotename}[1]{$\!\!\!$}%
    	\renewcommand{\fixmelogo}{}%
    	\hspace*{-0.35em}\raisebox{0.7em}[\height][\depth]
                {\\\makebox[0em][l]{\fxnote{\tiny{\color{myred}JR: }
                \textit{\color{mydarkgreen}#1}}}}%
    }
}
\let\jn=\jnote
\newcommand{\TOFIX}[1]{% using fixme
	\renewcommand{\fxnotename}[1]{$\!\!\!$}%
	\renewcommand{\fixmelogo}{}%
	{\fxfatal{\bf\normalsize\textit{\color{myred}#1}}}%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END newcommands for ignoring, commenting, ....
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> newcommands-labels-refs.tex <==
% label and ref newcommands
% now mostly deprecated (but redefined and kept for backward compatibility) - move to \cref from the cleveref package
\crefname{algocf}{alg.}{algs.}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefname{equation}{}{}
\Crefname{equation}{}{}

%DONE: xyzref{} should be able to handle multiple arguments so that you can
%reference multiple figures/equations at the same time -AG
%Now fixed with some package/command CREF.
\newcommand{\corrlabel}[1]{\label{corr:#1}}
\newcommand{\corrref}[1]{Corollary \ref{corr:#1}}
\newcommand{\assref}[1]{Assumption \ref{ass:#1}}
\newcommand{\asslabel}[1]{\label{ass:#1}}
%\newcommand{\eqnref}[1]{(\ref{eq:#1})}
%\newcommand{\eqnlabel}[1]{\label{eq:#1}}
\newcommand{\eqnlabel}[1]{\label{#1}}
\newcommand{\eqnref}[1]{\cref{#1}}
%\newcommand{\figlabel}[1]{\label{fig:#1}}
%\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\lstlabel}[1]{\label{lst:#1}}
\newcommand{\lstref}[1]{Listing~\ref{lst:#1}}
\newcommand{\figlabel}[1]{\label{#1}}
\newcommand{\figref}[1]{\cref{#1}}
\newcommand{\chaplabel}[1]{\label{chap:#1}}
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\exampleref}[1]{Example~\ref{ex:#1}}
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\tablabel}[1]{\label{#1}}
\newcommand{\tabref}[1]{\cref{#1}}
\newcommand{\thlabel}[1]{\label{th:#1}}
\newcommand{\thref}[1]{Theorem~\ref{th:#1}}
\newcommand{\thmlabel}[1]{\label{thm:#1}}
\newcommand{\thmref}[1]{Theorem \ref{thm:#1}}
\newcommand{\deflabel}[1]{\label{def:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\lemlabel}[1]{\label{lem:#1}}
\newcommand{\lemref}[1]{Lemma \ref{lem:#1}}
\newcommand{\examplelabel}[1]{\label{ex:#1}}
\newcommand{\labexample}[1]{\label{example:#1}}
\newcommand{\refexample}[1]{Example{ }\ref{example:#1}}
\newcommand{\httpref}[1]{}
\let\el=\eqnlabel
\let\er=\eqnref


==> newcommands-math.tex <==
%\newcommand{\ddt}[2]{{\frac{d}{d #2}\left. #1 \right.}}
\newcommand{\ddt}[2]{{\frac{d #1}{d #2}}}
\newcommand{\ddx}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand{\Ddx}[2]{{\frac{D}{d{#2}}\left[ #1 \right]}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\deq}{\triangleq}
\newcommand{\I}{I\left[\right]}
\newcommand{\ELL}[1]{L\left[#1\right]}
\newcommand{\w}{\omega}
\newcommand{\calD}{{\cal D}}
\renewcommand{\jmath}{j}
\newcommand{\Pinvt}{{P(t)}^{-1}}
\newcommand{\halmos}{\hskip\textwidth minus\textwidth \rule{6pt}{6pt}}
\newcommand{\calA}{{\cal A}}
\newcommand{\calAT}{{\cal A}^T}
\newcommand{\calL}{{\cal L}}
\newcommand{\calLadj}{\calL^\dagger}
\newcommand{\calR}{{\cal R}}
\newcommand{\Reals}{\Bbb{R}}
\newcommand{\Real}{\Bbb{R}}
\newcommand{\Safe}{\ensuremath{{\bf S}}}
\newcommand{\Pade}{{Pad\'e}}
\newcommand{\Complexes}{\Bbb{C}}
\newcommand{\HvecqLanc}{\Hvec^{(L)}_q}
\newcommand{\HvecqArn}{\Hvec^{(A)}_q}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\calDT}{{\cal D}^T}
\newcommand{\calCtil}{\tilde{\cal C}}
\newcommand{\calJtil}{\tilde{\cal J}}
\newcommand{\calDtil}{\tilde{\cal D}}
\newcommand{\JstarDphi}{J_{\Delta \phi}^*}
\newcommand{\Jstarphi}{J_{\phi}^*}
\newcommand{\vecbphi}{\vec b_{\phi}}
\newcommand{\vecbext}{\vec b_{\text{ext}}}
\newcommand{\phistarIdeal}{\phi_{\text{ideal}}^*}
\newcommand{\apdx}[1]{\appref{#1}} 
\newcommand{\delbydel}[2]{\ensuremath{\frac{\partial {#1}}{\partial {#2}}}}
\newcommand{\delbydeln}[3]{\ensuremath{\frac{\partial^{{#1}}
{#2}}{\partial{#3}^{{#1}}}}}
\newcommand{\delbydelat}[3]{\ensuremath{\left. \frac{\partial
{#1}}{\partial {#2}} \right|_{{#3}}}}
\newcommand{\dee}{\ensuremath{\mathrm{d}}}
\newcommand{\dbyd}[2]{\ensuremath{\frac{\mathrm{d} {#1}}{\mathrm{d}
{#2}}}}
\newcommand{\dbydn}[3]{\ensuremath{\frac{\mathrm{d}^{{#1}}{#2}}
{\mathrm{d}{#3}^{{#1}}}}}
\newcommand {\dist}[1] {{{\rm dist}\left({#1}\right)}}
\def\Matrix#1{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\textdiag}{{\text{diag}}}
\newcommand{\ihat}{\hat{\imath}}
\newcommand{\jhat}{\hat{\jmath}}
\newcommand{\khat}{\hat{k}}
\newcommand{\del}{\nabla}
\newcommand{\Rxx}{R_{\vec x \vec x}}
\newcommand{\Sxx}{S_{\vec x \vec x}}
\newcommand{\Snn}{S_{\vec n \vec n}}
\newcommand{\vecphi}{\vec \phi}
\newcommand{\Dphi}{\Delta \phi}
\newcommand{\vecDphi}{\vv{\Delta \phi}}
\newcommand{\dphi}{\delta \phi}
\newcommand{\vecdphi}{\vv{\delta \phi}}
\newcommand{\ah}{\alpha_g} % g for group
%\newcommand{\tDagger}{{\tilde t}}
\newcommand{\tDagger}{{t^{\!\dagger}}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\texthyphen}{\text{--}}

%The substack command can be used to produce a multi-line subscripts or superscripts:
%\sum_{\substack{0\le i\le m\\ 0<j<n}} P(i,j) produces a two-line subscript underneath the sum.
%A slightly more general form is the subarray environment which allows you to specify that each line should be left-aligned instead of centered, as here:
% \sum_{\begin{subarray}{l} i\in\Lambda\\ 0<j<n \end{subarray}} P(i,j) 

%\newcommand{\be}[1]{\begin{equation}\eqnlabel{#1}} % now moved to cleveref
\newcommand{\be}[1]{\begin{equation}\label{#1}}
\def\ee{\end{equation}}


==> newcommands-misc.tex <==
% Misc. commands
%\newcommand{\website}{http://www.eecs.berkeley.edu/\char126 jr/NOW-FT-Monograph/}

%\newcommand{\figdir}{./figures} % best to define this in the main tex file

% \newcommand{\bibdir}{.} % ditto

\newif\ifjournalsub
\newcommand{\ifthen}[2]{\ifthenelse{#1}{#2}{}}
\newcommand{\iftr}[1]{\boolean{#1}}

\newcommand{\DAEtoFSM}{ABCD}
\newcommand{\Brangluin}{Brangluin}
\newcommand{\LTIMORrefs}{pillage1,FeFr95a,OdCePiTCAD98,PhDaSiDAC2002,PhSiPMTBRDATE2004}
\newcommand{\nonlinearMORrefs}{RoTVPTCAS99,ReWhTCAD2003,PhTCAD2003,DoRoTCADPWP2008,
                               GuRoICCAD2008maniMOR}
\newcommand{\MORrefs}{\LTIMORrefs,\nonlinearMORrefs}
\newcommand{\proposalAcronym}{THz-PHLOGON}
\newcommand{\website}{http://www.eecs.berkeley.edu/$\sim$jr/NOW-FT-Monograph/}
\newcommand{\PNJLIM}{\textsf{\small PNJLIM}}
%\newcommand{\MATLAB}{\textbf{MATLAB}$^{\texttrademark}$}
\newcommand{\MATLAB}{MATLAB$^\text{\textregistered}$}

%%%% misc formatting setup
\newlength{\colwidth}
\newcommand{\pswidthcoeff}{0.9}
\newcommand{\psheightcoeff}{0.6}
\newlength{\pgwid}
% make LaTeX less fussy about line breaks, so that it typsets inline 
% math without overflowing -- perhaps remove if it causes trouble.
\sloppy 
\setcounter{secnumdepth}{5}  % numbered \paragraph == \subsubsubsection
\pagenumbering{arabic}
%\renewcommand{\thepage} {Body--\arabic{page}}
\hyphenation{op-tical net-works semi-conduc-tor} % correct bad hyphenation here



==> newcommands-squeeze-spaces.tex <==
\ignore{ TWEAKLIST OFTEN CAUSES ERRORS
%%% tweaklist renewcommands - 
\newcommand{\modifiedListParamters}{
  \setlength{\topsep}{0pt}%
  \setlength{\itemsep}{-0.1em}
  \setlength{\partopsep}{0em}
  \setlength{\parsep}{0em}
  \setlength{\leftmargin}{1.1em}
  \setlength{\itemindent}{0.0em}
}
\renewcommand{\enumhook}{
  \modifiedListParamters
  \setlength{\itemindent}{0.2em}
}
\renewcommand{\itemhook}{
  \modifiedListParamters
}
\renewcommand{\descripthook}{
  \modifiedListParamters
  \setlength{\itemindent}{-1.0em}
}
%%% end tweaklist renewcommands
}

% same functionality as tweaklist (but better?)
\let\labelindent\relax % to fix conflict with IEEEtran,otherwise not reqd?
\usepackage{enumitem}
\setenumerate{leftmargin=1em,itemindent=0em,labelindent=0em,itemsep=0em} % sets it globally.
% you can do it on a per list basis like this:
% \begin{enumerate}[leftmargin=1em,itemindent=0em,labelindent=0em,itemsep=0em]
%   \item ...
% \end{enumerate}


\ignore{not usually needed, but the definitions have useful info
		Space saving List environment for enumerations.

	\newcounter{myctr}
	\newenvironment{mylist}{\begin{list}{\arabic{myctr}.}
   		{\usecounter{myctr}
   		%\setlength{\topsep}{1mm}\setlength{\itemsep}{0.5mm}
   		\setlength{\topsep}{0.3mm}
   		\setlength{\itemsep}{0mm}
   		\setlength{\parsep}{0.3mm}
   		\setlength{\itemindent}{0mm}
   		\setlength{\partopsep}{0mm}
   		\setlength{\labelwidth}{15mm}
   		\setlength{\leftmargin}{4mm}
   		}
	}{\end{list}}

	\newenvironment{myitemize}{\begin{list}{$\bullet$}
	  \ignore{\setlength{\topsep}{0.8mm}\setlength{\itemsep}{0.25mm}}
	  {\setlength{\topsep}{1mm}\setlength{\itemsep}{0.25mm}
	  \setlength{\parsep}{0.1mm}
	  \setlength{\itemindent}{0mm}\setlength{\partopsep}{0mm}
	  \setlength{\labelwidth}{15mm}
	  \setlength{\leftmargin}{4mm}}
	}{\end{list}}
}

%%%% titlesec: squeezing whitespace between section headings
	\titlespacing{\section}{0pt}{*0}{*0.1} % {0pt} is indentation; {*0} is 
                                           % space above; {*0.5} is space below
	\titlespacing{\subsection}{0pt}{*0.1}{*0}
	\titlespacing{\subsubsection}{0pt}{*0.1}{*0}
%%%% end titlesec

%%%% squeezing whitespace in and around figures
    \floatsep=0em % space left between floats.
    \textfloatsep=0em % space between last top float or first bottom float and the text.
    \intextsep=0em % space left on top and bottom of an in-text float.
    %\dbltextfloatsep is \textfloatsep for 2 column output.
    %\dblfloatsep is \floatsep for 2 column output.
    \abovecaptionskip=0em % space above caption
    \belowcaptionskip=0em % space below caption
%%%% END squeezing whitespace in and around figures

\makeatletter
\g@addto@macro\normalsize{%
  \setlength\abovedisplayskip{1pt}
  \setlength\belowdisplayskip{1pt}
  \setlength\abovedisplayshortskip{1pt}
  \setlength\belowdisplayshortskip{1pt}
}
\makeatother

%\newcommand{\mycaption}[1]{\caption{\small #1}}
\newcommand{\mycaption}[1]{\caption{\tiny #1}}

% for captions spacing
\captionsetup[table]{font={scriptsize},format=hang,indention=0em}     %% change 1.2 as you like
\captionsetup[figure]{font={scriptsize},format=hang,indention=0em}    %% change as you like
 %% or
 %% \captionsetup{font={stretch=1.2}}  %% this affects both figure and table

% replace Figure x in captions by Fig. x
%\renewcommand{\figurename}{Fig.} % doesn't work.
%but \usepackage[figurename=Fig.]{caption} in packages-headers.tex does work.


%\renewcommand{\baselinestretch}{1.5}
%\setstretch{1.5}

%\def\baselinestretch{0.8593}\large\normalsize - this form works locally?
%\renewcommand{\baselinestretch}{0.94} - this form works only in the preamble
%\renewcommand{\baselinestretch}{0.90}
%\renewcommand{\baselinestretch}{0.5}
%\linespread{0.5} % 0.5 -> 7 lines per inch; 0.9 -> a bit more than 6 lines 
%                 % per vertical inch
% \linespread{0.99}

% baselinestretch fixes for squeezing. See also linespread
%\def\ssp{\def\baselinestretch{0.95645}\large\normalsize} % "single space"
%\def\ssp{\def\baselinestretch{0.905}\large\normalsize} % "single space"
\def\ssp{\def\baselinestretch{0.87}\large\normalsize} % "single space"
\def\dsp{\def\baselinestretch{1.3}\large\normalsize} % "double space"
\ssp

% indent paragraphs less (saves space)
\parindent 	1em
% do not indent paragraphs (saves more space)
\parindent 	0em
% adjust space between paragraphs (0em can obscure paragraph breaks)
\parskip 0.3em


==> newcommands-thm-env.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% theorem-like environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\EndProof{\hfill \quad \vrule width 1ex height 1ex depth 0pt  }
\newtheorem{corollary}{Corollary}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
%\newtheorem{illustration}{Illustration}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{defn}{Definition}[section]
\newtheorem{notation}{Notation}
\newtheorem{theorem}{Theorem}
\newenvironment{sketch}{\noindent{\bf Sketch of Proof}:}{\halmos}
\newenvironment{conjecture}{\noindent{\bf Conjecture}: \em}{}
\newcommand{\numberedtheorem}[3]{
	\ifthen{\not\equal{#1}{}}{
		\let\oof=\thetheorem
		\renewcommand{\thetheorem}{#1}
	}
	\begin{theorem}
	\ifthen{\not\equal{#2}{}}{
		\thmlabel{#2}
	}
	#3
	\end{theorem}
	\ifthen{\not\equal{#1}{}}{
		\let\thetheorem=\oof
		\addtocounter{theorem}{-1}
	}
}
\newcommand{\numberedlemma}[3]{
	\ifthen{\not\equal{#1}{}}{
		\let\oof=\thelemma
		\renewcommand{\thelemma}{#1}
	}
	\begin{lemma}
	\ifthen{\not\equal{#2}{}}{
		\lemlabel{#2}
	}
	#3
	\end{lemma}
	\ifthen{\not\equal{#1}{}}{
		\let\thelemma=\oof
		\addtocounter{lemma}{-1}
	}
}


==> package-and-newcommand-includes.tex <==
%%%%%%%%%%%%%%%%%% PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%
\RequirePackage{times}
%\RequirePackage[usenames]{pstcol} 
\RequirePackage[usenames]{pstricks} 

% Graphics (figures/images etc.)
%\usepackage[pdftex]{graphicx}
\RequirePackage{graphicx} % supplies \includegraphics
\graphicspath{{./octave-figures/}{./results/}{./figures/}{./snapshots/}}
\DeclareGraphicsExtensions{.eps,.pdf,.jpeg,.png}

\RequirePackage{rotating}
\RequirePackage{indentfirst} 
\RequirePackage{color} 
%\RequirePackage{picins} 
\RequirePackage{bmpsize} 
\RequirePackage{epsfig} % good old way of including figures
\RequirePackage{eepic} 
\RequirePackage{subfigure} % put figures side-by-side
\RequirePackage{wrapfig} % wrap text around figures
\RequirePackage{picinpar} % alternative to wrapfig, less useful

% Math (symbols/equations etc.)
\usepackage{cancel}
\RequirePackage{amsmath,amssymb,amsbsy,amsfonts,dotlessj} 
\RequirePackage{latexsym}
\RequirePackage{mathptm} % - AG (Don't like \mathcal{C} that this produces
\RequirePackage{mathptmx} % times (smaller) math fonts, greek characters also italicized
\RequirePackage{bm} % boldmath
\DeclareMathVersion{bold} 

% Formatting
\RequirePackage{multicol}
\RequirePackage{esvect} % defines \vv{}
\RequirePackage{ifthen}
\RequirePackage{etoolbox}
\RequirePackage{relsize}
\RequirePackage{soul}   % Provides \hl{some-text}
%\RequirePackage{showkeys} 
%\RequirePackage[final,notref]{showkeys} 
%\RequirePackage[top=0.8cm,bottom=0.8cm,left=0.8cm,right=0.8cm,nohead,nofoot]{geometry}
%\RequirePackage[top=1.2cm,bottom=1.3cm,left=1.2cm,right=1.2cm,nohead,nofoot]{geometry}

\usepackage[nolist,nohyperlinks]{acronym}
\RequirePackage{setspace}
\RequirePackage{moreverb}
\RequirePackage{ulem} % provides \uline
        \let\em=\it % ulem package redefines \em=\uline
\RequirePackage[sectionbib]{chapterbib}
\RequirePackage{fancyhdr}
\RequirePackage{array}
\RequirePackage{floatflt} % does (to some extent) work inside itemize environment %
                          % use \fltditem, see $LATEXDOCS/floatflt.pdf, esp. Sec 3.1
\RequirePackage{srcltx}
\RequirePackage{chemarrow}

% Utilities
\RequirePackage{todonotes}
\RequirePackage{tcolorbox}
\RequirePackage{fixme}
\RequirePackage[footnotesize,bf,figurename=Fig.,hang]{caption}
%\usepackage[scriptsize,hang,bf]{caption}
%\RequirePackage[hypertex]{hyperref} 
\RequirePackage{hyperref} 
%\definecolor{linkColor}{rgb}{0.1,0.1,0.8}
%\usepackage[colorlinks=true,bookmarks,pdfpagemode=UseOutlines,linkcolor=linkColor,citecolor=linkColor,pagecolor=blue,urlcolor=blue,pdftitle={Verification, Learning, Control},pdfauthor={Jaijeet Roychowdhury},plainpages=false]{hyperref}

%\usepackage{./tweaklist} % allow changing of item spacings in standard itemize,
                         % enumerate, description environments
					     %%% tweaklist: compress lists. Also check out 
                         %%% \usepackage{mdwlist} (use itemize*, enumerate*, 
                         %%% description* with that)
                         % enumhook for the enumerate environment, itemhook for
                         % the itemize environment, and descripthook for the
                         % description environment.
                         % HOWEVER, CAUSES ERRORS. Use enumitem instead.

% enumitem package included from newcommands-squeeze-spaces.tex

\providecommand{\subparagraph}{} % needed for IEEEtran.cls (which does not define subparagraph); \providecommand checks if it is already defined
\RequirePackage[small,compact]{titlesec} % squeezing whitespace between section heading
\RequirePackage[sectionbib,square,sort&compress,numbers]{natbib} % needed for IEEEtran; but proposal.cls pulls it in automatically
%\RequirePackage{cite} % natbib doesn't like this
\RequirePackage{lipsum}
\RequirePackage{microtype}
\RequirePackage{url}
\RequirePackage{listings} % Required for insertion of code
\RequirePackage{multirow}
\RequirePackage{booktabs}
% load cleveref last, but before algorithm2e (which breaks cleveref)
\RequirePackage[compress,capitalise,noabbrev]{cleveref} % defines \cref, \Cref, etc; options are compress (don't sort), sort (don't compress), sort&compress (default), nosort (neither sort nor compress)
%\RequirePackage{algorithmic}
%\RequirePackage{algorithm}
%\RequirePackage[boxed,algoruled]{algorithm2e}
\RequirePackage[boxed,algoruled,linesnumbered,vlined,nofillcomment]{algorithm2e}
%\usepackage[yyyymmdd,hhmmss]{datetime} % use: Compiled on \today\ at \currenttime
\usepackage{datetime2} % ]use: Compiled on \DTMnow. And do \documentstyle[pacific]{...}

%%%%%%%%%%%%%%%%%% END PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%

% fixme package setup
\fxsetup{ status=draft,
		  %author={\tiny JR},
	  	  layout=footnote,
		  layout=inline, % also try footnote or pdfnote
		  theme=color,
	  	  marginclue
}
\definecolor{mydarkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{myred}{rgb}{0.9,0.0,0.0}
%\definecolor{fxnote}{rgb}{0.8000,0.0000,0.0000}
\renewcommand{\englishlistfixmename}{List of changes needed}
% Decrease spacing between items in bib
\newcommand{\BIBdecl}{\setlength{\itemsep}{0.25 em}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Multi-column the bib
%\patchcmd{\thebibliography}
%  {\list}
%  {\begin{multicols}{2}\list}
%    {}
%    {}
%\appto{\endthebibliography}{\end{multicols}}

%------------------------------------------------------------------------------
%   CODE INCLUSION CONFIGURATION
%------------------------------------------------------------------------------

\lstloadlanguages{Matlab}
\lstset{language=Matlab,
        frame=single, % Single frame around code
        basicstyle=\scriptsize\ttfamily,
        % keywordstyle=[1]\color{blue}\bf, % Perl functions bold and blue
        keywordstyle=[3]\color{blue}\underbar, % Custom functions underlined and blue
        identifierstyle=, % Nothing special about identifiers                                         
        commentstyle=\usefont{T1}{pcr}{m}{sl}\color{green}\scriptsize, 
            % Comments are in small dark green courier font
        stringstyle=\color{red}, 
        showstringspaces=false, % Don't put marks in string spaces
        tabsize=4, % 5 spaces per tab
        % 
        % Put standard functions not included in the default language here
        %morekeywords={rand},
        % Put function parameters here
        %morekeywords=[2]{on, off, interp},
        % Put user defined functions here
        %morekeywords=[3]{test},
        %
        morecomment=[l][\color{blue}]{...}, % Line continuation (...) like blue comment
        % numbers=left, % Line numbers on left
        % firstnumber=1, % Line numbers start with line 1
        % numberstyle=\tiny\color{blue}, % Line numbers are blue and small
        % stepnumber=5 % Line numbers go in steps of 5
}

% Creates a new command to include an Matlab script, the first parameter is the
% filename of the script (without .pl), the second parameter is the caption
\newcommand{\matlabscript}[2]{
    \begin{itemize}
    \item[]\lstinputlisting[caption=#2,label=#1]{#1}
    \end{itemize}
}

\input colour-defs
\input newcommands-highlight-ignore-comments-annotations
\input newcommands-labels-refs
\input newcommands-eg-ie-etc
\input newcommands-for-bibtex % BP, BPnom, IP, presenter, putDOI, DP, etc
\input newcommands-misc
\input newcommands-squeeze-spaces
\input newcommands-math
% \input newcommands-thm-env



